A Practical Mixed Precision Algorithm for Post-Training Quantization

Neural network quantization is frequently used to optimize model size, latency and power consumption for on-device deployment of neural networks. In many cases, a target bit-width is set for an entire network, meaning every layer get quantized to the same number of bits. However, for many networks some layers are significantly more robust to quantization noise than others, leaving an important axis of improvement unused. As many hardware solutions provide multiple different bit-width settings, mixed-precision quantization has emerged as a promising solution to find a better performance-efficiency trade-off than homogeneous quantization. However, most existing mixed precision algorithms are rather difficult to use for practitioners as they require access to the training data, have many hyper-parameters to tune or even depend on end-to-end retraining of the entire model. In this work, we present a simple post-training mixed precision algorithm that only requires a small unlabeled calibration dataset to automatically select suitable bit-widths for each layer for desirable on-device performance. Our algorithm requires no hyper-parameter tuning, is robust to data variation and takes into account practical hardware deployment constraints making it a great candidate for practical use. We experimentally validate our proposed method on several computer vision tasks, natural language processing tasks and many different networks, and show that we can find mixed precision networks that provide a better trade-off between accuracy and efficiency than their homogeneous bit-width equivalents.

==> sections/03_method.tex <==
\section{Method}

In this section we introduce our two-phase algorithm to solve the problem of mixed precision quantization in the post-training quantization setting. In the first phase, we create a per-layer sensitivity list by measuring the loss of the entire network with different quantization options for each layer. This list gives an estimate of the impact of quantizing for a layer on the network's performance. The second phase of the algorithm starts with the entire network quantized to the highest possible bit-width, after which based on the sensitivity list created in phase 1, we iteratively flip the least sensitive quantizers to lower bit-width options untill the performance budget is met or our accuracy requirement gets violated. 

As discussed in the later sections, labels have no role in creating the per-layer sensitivity list obtained in phase 1 of our method, making the algorithm agnostic to the category of the data used for calibration. Also, due to the simple iterative nature of phase 2 of our algorithm, our method seamlessly allows a user to pick either an on-device accuracy target or a performance budget by incorporating practical hardware deployment constraints in the search.

\subsection{Preliminaries}
In neural network quantization, real valued weight $W^{r}$ and activation tensors $x^{r}$ are quantized to an appropriate low precision value. The quantization operation for a $b$-bit uniform quantizer $q_{b}$ is defined as

\begin{align}
    W_{int} &= Clip \left( \nint[\Big]{\frac{W^{r}}{s}}, n, p \right) \\
    W^{r} &\approx q_{b}(W^{r}) = sW_{int} \hfill
\end{align}
% \begin{equation}
% \!
%     \begin{split}
%     W_{int} &= q_{b}(W^{r}) &= Clip \Big( \nint[\Big]{\frac{W^{r}}{s_{x}}}, n, p \Big) \\
%    
%     W \thickapprox &= s_{x}W_{int} \hfill
%   \end{split}
% \end{equation}
where $s$ denotes the quantization scale parameter and, $n$ and $p$ denote the negative and positive integer thresholds for clipping. The same principle holds for per-channel scheme of quantization \cite{krishnamoorthi2018quantizing}, for which the scale factor $s$ is a vector with each value representing scale of each individual channel. For a more detailed coverage, please refer to \citet{nagel2021white}.

\subsection{Phase 1: Generating Sensitivity List}
In order to perform mixed precision quantization on a pretrained neural network, it is important to understand the effect of quantizing a layer on the network's performance. The first phase of our algorithm aims at creating such a per-layer sensitivity list. This list captures the relative sensitivity of layers to quantization, without taking into account any correlations with other layers for efficiency.
% The idea of this list is that it captures the effect of quantizing a layer on the network's final loss. 

Next to the accuracy of the estimate of this list, for practical use-cases there are two more important factors for the creation of this list; the run-time of the algorithm, and the amount of data necessary to make a good estimate. In this section we propose to use the signal to quantization noise ratio (SQNR) as a metric to measure the relative sensitivity of each quantizer $q$ when quantized to different bit-width options $b \in B$. For a converged pre-trained network, quantizing the network introduces noise at the output which increases the network loss and directly affects the logits and the task performance. Hence, in order to measure the sensitivity to quantization of each quantizer $q$ in the network,  we define,
% \begin{equation}\label{e:SQNR} 
%     \Omega_{q,b}^{SQNR} = 10\log \frac{1}{N} \sum_{i=1}^{N} \frac{  \int_{}^{}s^{2}f(s)ds}{\int_{}^{}e^{2}f(s)ds}
% \end{equation}
\begin{equation}\label{e:SQNR} 
    %\Omega_{q,b}^{SQNR} = 10\log \frac{\mathbb{E}[s^{2}]}{\mathbb{E}[e^{2}]}
    \Omega_{q,b}^{SQNR} = 10\log \frac{1}{N}\sum_{i=1}^{N}\frac{\mathbb{E}[{F}_{\theta} (x_{i})^{2}]}{\mathbb{E}[e(x_{i})^{2}]}
\end{equation}
where, $\Omega_{q,b}^{SQNR}$ is the average SQNR at the output of the network using N calibration data points, and the quantization error
% \begin{equation}
%     s = {F}_{\theta} (x)
% \end{equation}
\begin{equation}
   e(x) = \mathcal{F}_{\theta} (x) - \mathcal{Q}_{q,b}(\mathcal{F}_{\theta} (x))
\end{equation}
  where $\mathcal{F}_{\theta}$ represents the full precision network and $\mathcal{Q}_{q,b}(\mathcal{F}_{\theta})$ represents the quantized network with the quantizer $q$ set to bit-width $b$ and rest of the layers and activations in full precision.
\\

% Unlike accuracy or other task performance metrics, SQNR measured at the output, $\Omega_{q,b}^{SQNR}$, does not depend on labels or category of the input images. This makes the approach robust to the quality of available data by making it agnostic to labels.

\subsection{Phase 2: Finding Mixed Precision Configuration}
Once we have the relative sensitivity of layers to quantization, the next challenge is to allocate bit-widths to each layer in the network for the desired performance budget. To solve this optimization problem in an efficient manner, we propose to use an iterative pareto frontier based approach in the phase 2 of our algorithm to obtain a network with best performance-efficiency trade-off meeting the performance criteria. 

Phase 2 of our algorithm starts with the entire network quantized to a baseline highest bit-width that gives the best task performance upon quantization. At each step, in-order to minimize the loss we incur due to reducing the precision of a quantizer to a lower bit-width, we use the sensitivity list to get the best candidate for minimizing this performance loss vs efficiency gain trade-off. This pareto frontier based approach allows us to search for the most efficient mixed precision configuration meeting the performance budget. The approach is greedy, but works very well in practice.

\begin{algorithm}[!ht]
  \textbf{Input}: Network with full precision quantizer $\left\{q_{l} \right \} _{l=1}^{L}$, bit-width candidates for mixed precision $\left\{b_{i}\right \} _{i=1}^{N}$, Performance budget $\gamma$ and evaluation criteria $\mathcal{E}$
  \\
  
  \textbf{Output}: Network with quantized quantizer $\left\{q_{l}^{Q} \right \} _{l=1}^{L}$ and corresponding bit-width allocations $\left\{b^{l}\right \} _{l=1}^{L}$
  \\
  
%   \textbf{Phase 0}: Define baseline bit-width candidate 
%   \\
  
%   $b_{baseline}$ = $\underset{b}{\arg\max}$
  \textbf{Phase 1}: 
  \\
  Initialize Sensitivity list $S$
  \\
  
  \For{quantizer q $\in \left\{q_{i}\right\}_{i=1}^{L}$}
    {
    \For{bit-width b $\in B - \left\{b_{baseline}\right\}$ }
        {
        Calculate $\Omega_{q,b}^{SQNR}$  \\
        Add $(q, b, \Omega_{q,b}^{SQNR})$ to $S$
        }
    }
  \\    
  Sort sensitivity list $S$ (highest to lowest $\Omega_{q,b}^{SQNR}$)
  \\
  
  \textbf{Phase 2}: 
  \\
  Initialize network to baseline candidate\\
  Performance $\mathcal{P} = \mathcal{E}(network)$
  \\
  
  \For{$q,b \in S$}
  {
    
    Quantize $q$ to bit-width $b$\\
    Update $\mathcal{P} = \mathcal{E}(network)$
    
  \If{$\mathcal{P} < \gamma$}
    {
        return previous model
    }
  }\\
  
\caption{Post-Training Mixed Precision Algorithm}
\end{algorithm}
\\

We define two budget criteria relevant to on-device deployment of neural networks that can be easily used with our mixed precision routine.
\subsubsection{Efficiency based budget:} Quantizing a network to lower bit-widths improves the latency and power consumption, hence improving the overall efficiency of the model when deployed on-device. In-order to measure efficiency of a mixed precision network independent of a specific target platform, we use Bit Operations (BOPs)~\cite{van2020bayesian} as a surrogate measure. BOPs are defined as:
\begin{equation}
   BOPS(\phi) = \sum_{ops_{i} \in network} bits(\phi_{i})MAC(op_{i})
\end{equation}
where $op_{i}$ represents operations in the network, $bits(\phi_{i})$ the bit-width associated with weights and activations for operation $op_{i}$ and $MAC(op_{i})$ represents the total of Multiply-Accumulate (MAC) operations for operation $op_{i}$. As discussed in \cite{van2022simulated}, Bits Operations (BOPs) correlates strongly with relative power consumption and hence a budget on BOPs can be used as a criteria to obtain a desirable efficiency target.

\subsubsection{Task Performance based budget:} For practical use-cases, achieving certain task performance can be used as a criteria to obtain a mixed precision network. A user can define the lowest performance of the network they would tolerate, and find the best bit-width setting to get the best on-device performance while allowing no more than their maximal tolerated degradation in performance. 
% \subsubsection{Noise based budget:} Quantizing layers of a neural network to lower bit-width introduces quantization noise which affects the local output feature map of the that layer. This noise propagates through the network and also effects the final output feature map which directly affects the task performance. Hence, threshold on tolerable noise at the output can be used as a criteria to obtain a mixed precision configuration.

% As both the task performance and memory footprint of the network, increase monotonically with increase in BOPs of the model, these two criteria fit well with our pareto frontier based approach to return the least BOPs model meeting the budget target.

\subsection{Quantizer Groups in networks}
As described in the previous section, current methods in the mixed precision literature consider all weight layers and activations to be independent. This is generally not the case in practice. Not all options for quantizing operations in the network might be available. For example, a device might have only implemented kernels for W4A8, 4 bit weights and 8 bit activations, and W8A16, 8 bit weights and 16 bit activations. This creates a dependency for the specific kernels that can be picked by the mixed-precision algorithm. In this example, 4 bit weights always come with 8 bit activations, and 8 bit weights come with 16 bit activations. And other solutions are not valid.
To incorporate these practical constraints in our algorithm, we introduce the concept of a Quantizer Group which are groups of weights and activations connected through shared operations in a computational graph. To ensure these shared operations in a group are performed in a certain bit-width on-device, we constraint inputs to all the operation to be quantized to the same precision.

Incorporating the concept of quantizer groups in the current search based mixed precision \cite{huang2022sdq, yang2021fracbits} and metric based mixed precision methods \cite{dong2019hawq, ma2021ompq} can be non-trivial due to the design and computational complexity of the algorithms. Due to the iterative nature of our method, we can easily incorporate this practical constraint in our algorithm by measuring the per-group sensitivity and flipping the entire quantizer group instead of individual quantizers at each step of our phase 2.

\subsection{Improving post-training Mixed Precision for Low Bit Quantization with AdaRound}
For low bit ($<$8) quantization, it is very important to correctly capture the weight-activation quantization trade-off to obtain an optimal mixed precision configuration. AdaRound \cite{nagel2020up}, a post-training quantization algorithm which learns better rounding for weight quantization, has proven to be very effective in practice to improve low bit weight quantization performance of neural networks. Hence, in-order to improve the performance of our mixed precision method, we propose to integrate AdaRound into our algorithm.

% Proposal Markus, not best yet, feel free to improve
To incorporate AdaRound, we propose to use AdaRounded weights to create the per-layer sensitivity of layers in Phase 1 of our algorithm. This allows us to obtain a sensitivity list with AdaRound and captures the correct trade-off between weight and activation quantization.
Due to the sequential and layer-wise optimization of the AdaRound algorithm, we can reuse the AdaRounded weights from Phase 1 and stitch the per-layer rounded weights together for each bit-width configuration we test in Phase 2. 
This allows to add AdaRound seamlessly into our mixed precision algorithm with minimal compute overhead. We will show this is very effective in improving the mixed precision network's performance.

% Org paragraph
% This allows us to obtain an improved sensitivity list which is AdaRound-awar. Next, due to the sequential and layer-wise optimization nature of the AdaRound algorithm, we stitch AdaRounded layers together based on the bit-width allocated to every layer to obtain an improved mixed precision network at each iteration of our Phase 2. Due to the fact that models optimized through the AdaRound routine can be seamlessly stitched together with minimal overall compute overhead, our proposed enhancement can very efficiently be used to improve performance of a mixed precision network to achieve better on-device performance. 



% Both the improvements are summarized in algorithm \ref{adaround-mp}.

% \begin{algorithm}[!ht]

%   \textbf{Initialization}: Perform AdaRound on the input network for each unique weight bit-width $b_{w} \in B$ to obtain optimized networks with AdaRounded quantizers $\left\{q^{b_{w}}_{l} \right \} _{l=1}^{L}$
%   \\
  
%   \textbf{Phase 1}: 
%   \\
%   Initialize Sensitivity list $S$
%   \\
  
%   \For{quantizer q $\in \left\{q_{i}\right\}_{i=1}^{L}$}
%     {
%     \For{bit-width b $\in B - \left\{b_{baseline}\right\}$ }
%         {
%         Calculate $\Omega_{q^{b},b}^{SQNR}$  \\
%         Add $(q^{b}, b, \Omega_{q^{b},b}^{SQNR})$ to $S$
%         }
%     }
%     Sort sensitivity list $S$ (highest to lowest $\Omega_{q,b}^{SQNR}$)
%   \\
  
%   \textbf{Phase 2}: 
%   Initialize network to baseline bit-width AdaRounded model\\
%   Performance $\mathcal{P} = \mathcal{E}(network)$
%   \\
  
%   \For{$q,b \in S$}
%   {
    
%     Replace quantizer $q$ with AdaRounded quantizer $q^{b}$\\
%     Update $\mathcal{P} = \mathcal{E}(network)$
    
%   \If{$\mathcal{P} < \gamma$}
%     {
%         return previous model
%     }
%   }\\
  
% \caption{AdaRound-aware Phase 1 and 2}
% \label{adaround-mp}
% \end{algorithm}


% \begin{algorithm}[!ht]

%   \textbf{Initialization}: Perform AdaRound on the input network for each unique weight bit-width $b_{w} \in B$ to obtain optimized networks with AdaRounded quantizers $\left\{q^{b_{w}}_{l} \right \} _{l=1}^{L}$
%   \\
  
  
  
% \caption{AdaRound Integrated Phase 2}
% \end{algorithm}

% Due to the sequential and layer wise optimization nature of the AdaRound algorithm, models optimized through the AdaRound routine can be seamlessly stitched together improving the performance of mixed precision networks without any additional compute overhead. Also, as discussed by Nagel et al \cite{nagel2020up}, AdaRound due to its label free approach and robustness to images used for optimization, makes it an ideal choice for integration with our pipeline.


% \begin{table*}
%     % \addtolength{\tabcolsep}{-2pt}
%     \fontsize{10pt}{10pt}\selectfont 
%     \centering
%     \begin{tabular} { | p {3.5 cm} | p {1.5 cm} | p {1.5 cm} |p {1.5 cm} |p {1.5 cm} | p {1.5 cm} | }
    
%     \hline
%     Model & FP32 & W8A8 ($r$=0.5) &  PTQ MP ($r$=0.5) &  W6A8 ($r$=0.375) & PTQ MP ($r$=0.375)\\
%     \hline
%     % \multicolumn{2} { | c | }{Rel. BOPs wrt W8A16 (r) } &  \multicolumn{1} { | c | }{$r$= 1}  &  \multicolumn{1} { | c | }{$r$= 0.5}  &  \multicolumn{1} { | c | }{$r$= 0.375}  &  \multicolumn{1} { | c | }{$r$= 0.25} \\
%     % \hline:q
     
%     Mobilenetv3 & $74.04\%$ & $68.75\%$ & $71.65\%$ &$65.20\%$ &  $66.70\%$ \\

%     Deeplabv3-mobilenetv3 & $0.6887$ &  $0.5784$ & $0.6700$ & $0.535$ & $0.669$ \\
    
%     Efficientnet-b0 & $77.67\%$ &  $12.40\%$ & $74.28\%$ & $12.62\%$ & $61.30\%$\\
    
%     BERT (MNLI) & $84.40\%$ &  $74.13\%$ & $82.97\%$ & $75.65\%$ & $82.22\%$\\


%     Efficientnet-lite & $75.44\%$ &  $75.13\%$ & $75.14\%$ & $73.43\%$ & $73.64\%$\\

%     Mobilenetv2 & $71.87\%$ & $70.44\%$ & $70.68\%$ & $68.14\%$ &  $67.38\%$\\

%     Resnet50 & $76.13\%$ & $75.95\%$ & $75.95\%$ & $75.41\%$ & $74.98\%$\\

%     Resnet18 & $69.75\%$ & $69.56\%$ & $69.56\%$ & $69.27\%$ & $67.39\%$\\
    

%     \hline

% \end{tabular}
%     \caption{MP using W4A8, W8A8 and W8A16 bit-width candidates. Comparison between fixed precision quantization and mixed precision quantization}
%     \label{tab:fixed-vs-mixed}
% \end{table*}

\begin{table*}
    % \addtolength{\tabcolsep}{-2pt}
    \centering
    \begin{tabular} {  lccccc }
    \toprule
    Model & FP32 & W8A8 &  PTQ MP &  W6A8  & PTQ MP\\
    &   &  ($r$=0.50) &  ($r$=0.50) &   ($r$=0.375)  &  ($r$=0.375)\\

    \midrule
    Resnet18 & $69.75\%$ & $69.56\%$ & $69.56\%$ & $69.27\%$ & $67.39\%$\\
    Resnet50 & $76.13\%$ & $75.95\%$ & $75.95\%$ & $75.41\%$ & $74.98\%$\\
    Mobilenetv2 & $71.87\%$ & $70.44\%$ & $70.68\%$ & $68.14\%$ &  $67.38\%$\\
    Mobilenetv3 & $74.04\%$ & $68.75\%$ & $71.65\%$ &$65.20\%$ &  $66.70\%$ \\
    Efficientnet-lite & $75.44\%$ &  $75.13\%$ & $75.14\%$ & $73.43\%$ & $73.64\%$\\
    Efficientnet-b0 & $77.67\%$ &  $12.40\%$ & $74.28\%$ & $12.62\%$ & $61.30\%$\\
    Deeplabv3-mobilenetv3 & $0.6887$ &  $0.5784$ & $0.6700$ & $0.5350$ & $0.6690$ \\
    BERT (MNLI) & $84.40\%$ &  $74.13\%$ & $82.97\%$ & $75.65\%$ & $82.22\%$\\
    ViT & $81.31\%$ &  $18.83\%$ & $80.58\%$ & $16.37\%$ & $77.08\%$\\

    \bottomrule
\end{tabular}
    \caption{MP using W4A8, W8A8, W8A16 bit-width candidates. Comparison between fixed precision quantization and mixed precision quantization.}
    \label{tab:fixed-vs-mixed}
\end{table*}

\begin{table*}
    % \addtolength{\tabcolsep}{-2pt}
    % \fontsize{10pt}{10pt}\selectfont 
    \centering
    \begin{tabular} {  lccccc }
    \toprule
    Model & FP32 & W6A6  & PTQ MP &  W4A8   &  PTQ MP \\
          &   &  ($r$=0.281) &  ($r$=0.281) &   ($r$=0.25)  &  ($r$=0.25)\\
    \midrule
    Resnet18 & $69.75\%$ & $66.09\%$ & $65.14\%$ & $54.93\%$ & $63.14\%$ \\
    Resnet50 & $76.13\%$ & $70.54\%$ & $73.11\%$ & $66.82\%$ & $73.05\%$ \\
    Efficientnet-lite & $75.44\%$ &  $72.87\%$ & $74.17\%$ & $6.37\%$ & $73.49\%$\\
    Mobilenetv2 & $71.87\%$ & $58.60\%$ & $64.97\%$ & $9.55\%$ & $61.81\%$ \\
    Mobilenetv3 & $74.04\%$ & $4.19\%$ & $42.57\%$  & $2.83\%$ & $28.67\%$ \\

    \bottomrule
\end{tabular}
    \caption{MP using expanded search space: W4A4, W4A6, W6A4, W6A6, W8A6, W6A8, W8A8, W8A16 bit-width candidates. Comparison between fixed precision quantization and mixed precision quantization for low bit-widths.}
    \label{tab:fixed-vs-mixed_expanded}
\end{table*}


% \begin{table*}
%     % \addtolength{\tabcolsep}{-2pt}
%     \fontsize{10pt}{10pt}\selectfont 
%     \centering
%     \begin{tabular} { | p {3.5 cm} | p {1.5 cm} | p {1.5 cm} |p {1.5 cm} |p {1.5 cm} | p {1.5 cm} | }
%     \hline
%     Model & FP32 & W6A6 ($r$=0.281) & PTQ MP ($r$=0.281) &  W4A8 ($r$=0.25)  &  PTQ MP ($r$=0.25)\\
%     \hline
%     % \multicolumn{2} { | c | }{Rel. BOPs wrt W8A16 (r) } &  \multicolumn{1} { | c | }{$r$= 1}  &  \multicolumn{1} { | c | }{$r$= 0.5}  &  \multicolumn{1} { | c | }{$r$= 0.375}  &  \multicolumn{1} { | c | }{$r$= 0.25} \\
%     % \hline
     
%     Mobilenetv3 & $74.04\%$ & $4.19\%$ & $42.57\%$  & $2.83\%$ & $28.67\%$ \\

%     Efficientnet-lite & $75.44\%$ &  $72.87\%$ & $74.17\%$ & $6.37\%$ & $73.49\%$\\

%     Mobilenetv2 & $71.87\%$ & 58.60$\%$ & $64.97\%$ & $9.55\%$ &$61.81\%$ \\

%     Resnet50 & $76.13\%$ & $70.54\%$ & $73.11\%$ & $66.82\%$ & $73.05\%$\\

%     Resnet18 & $69.75\%$ & $66.09\%$ & $65.14\%$ & $54.93\%$ & $63.14\%$\\
    

%     \hline

% \end{tabular}
%     \caption{MP using expanded search space: W4A4, W4A6, W6A4, W6A6, W8A6, W6A8, W8A8, W8A16 bit-width candidates. Comparison between fixed precision quantization and mixed precision quantization for low bit-widths}
%     \label{tab:fixed-vs-mixed_expanded}
% \end{table*}


\subsection{Improving Phase 2 mixed precision configuration search}
Due to the sequential nature of our phase 2 algorithm, the overall run-time complexity to search for a desired mixed precision configuration is $\mathcal{O}(LM)$, where $L$ is the depth of the network and $M$ is the number of bit-width options for mixed precision. In-order to improve the run-time of our search algorithm, we propose to use  improved binary search based scheme exploiting the monotonic nature of the pareto curve obtained in phase 2.



We start with a basic binary search  \cite{knuth1997art}, which reduces the overall search run-time complexity to $\mathcal{O}\left(\log_2(LM)\right)$. We further consider given the nonlinear nature of the pareto curve, first use base binary search to divide the entire curve into several piece-wise linear sub curves. For the linear sub curve, an interpolation search \cite{peterson1957addressing} can be employed to further reduce the search candidate to 1. In implementation, we use 2 times of binary search to divide the entire $LM$-points pareto curve to 4 $\lceil LM/4\rceil$-points sub curve candidates, then do the interpolation search on one of the candidate. Our improved hybrid search is illustrated in Figure \ref{fig:hybridsearch}.

\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.38\textwidth]{figures/Binary+interp.png}} 

    \caption{ Illustration of Binary + Interpolation Search.}
    \label{fig:hybridsearch}
\end{figure}
% \begin{algorithm}[!ht]
%   \textbf{Binary Search 1}: \\ 
%   Compute $\mathcal{P}_1 = \mathcal{E}(network)$ for quantizer q $\in \left\{q_{i}\riSht\}_{i=1}^{\lceil L/2\rceil}$ to bit-width $b$\\
%   \textbf{Binary search 2}: \\
%   \If {$\mathcal{P}_1 < \gamma$}
%   {
%   Compute $\mathcal{P}_2 = \mathcal{E}(network)$ for quantizer q $\in \left\{q_{i}\right\}_{i=1}^{\lceil L/4\rceil}$ to bit-width $b$\\
%     \If{$\mathcal{P}_2 < \gamma$}
%     {
%      $\mathcal{P}_3 = \mathcal{P}_{baseline}$ \\
%      go to Interpolation Search for $i\in\left{[}1, \lceil L/4\rceil\right{]}$
%     }
%     \Else
%     {
%     go to Interpolation Search for $i\in\left{[}\lceil L/4\rceil, \lceil L/2\rceil\right{]}$
%     }
%   }
%   \Else
%   {
%   Compute $\mathcal{P}_2 = \mathcal{E}(network)$ for quantizer q $\in \left\{q_{i}\right\}_{i=1}^{\lceil 3L/4\rceil}$ to bit-width $b$\\
%     \If{$\mathcal{P}_2 < \gamma$}
%     {
%      go to Interpolation Search for $i\in\left{[}\lceil L/2\rceil, \lceil 3L/4\rceil\right{]}$
%     }
%     \Else
%     {
%     $\mathcal{P}_3 = \mathcal{E}(network)$ for quantizer q $\in \left\{q_{i}\right\}_{i=1}^{\lceil L\rceil}$ to bit-width $b$ \\
%     go to Interpolation Search for $i\in\left{[}\lceil 3L/4\rceil, L\right{]}$
%     }
%   }
  
%   \textbf{Interpolation Search}: 
%   \\
%   Do interpolation search in the region from Binary Search 2
%   \\
  
% \caption{Binary + Interpolation Search}
% \label{alg:hybridsearch}
% \end{algorithm}



==> sections/04_results.tex <==
\section{Results}
\subsection{Comparison to Fixed Precision Quantization}
In this section we compare our mixed precision results with fixed single precision quantization. For our experiments, we use AI Model Efficiency Toolkit (AIMET) \cite{aimet,siddegowda2022neural} to quantize the models to desired bit-widths and use the per channel weight quantization and symmetric and asymmetric schemes for weight and activation tensors. For quantization range setting for each quantizer, we use MSE based criteria to set the min-max ranges. 

In figure 6, We compare our PTQ mixed precision algorithm to fixed precision quantization using most widely used bitwidth search space (W4A8, W8A8 and W8A16) for on device deployment. We expand our search space to 6 and 4 bits for weights and activations and compare our mixed precision algorithm to fixed precision quantization as shown in figure 7. In most usecases, at a similar relative BOPs value,
our mixed precision solution outperforms or performs at par with single precision quantized network achieving a better performance-latency tradeoff.

\subsection{Compression based Mixed Precision}
Table 1 compares task performance of various mixed precision configurations of networks based on compression measured as relative BOPs with respect to W8A16 model. Our AdaRound integrated mixed precision algorithm out performs similar relative BOPs fixed precision quantized models in most cases giving a better accuracy vs latency trade-off. For all the experiments, only 256 label free task images were used both for AdaRound optimization and sensitivity calculation in phase 1, demonstrating effectiveness of our method in presence of less data.

\begin{table}[H]
    \addtolength{\tabcolsep}{-2pt}
    \fontsize{6.5pt}{6.5pt}\selectfont
    \centering
    \begin{tabular} { | p {1.5 cm} | p {0.8 cm} | p {1.0 cm} | p {0.75 cm} | p {1.1 cm} | p {0.95 cm} | }
    \hline
    
    \multicolumn{6} { | c | }{Fixed Precision Quantization}\\
    \hline
    Model & FP32 & W8A16 & W8A8 & W6A8 & W4A8\\
    \hline
    \multicolumn{2} { | c | }{Rel. BOPs wrt W8A16 (r) } &  \multicolumn{1} { | c | }{$r$= 1}  &  \multicolumn{1} { | c | }{$r$= 0.5}  &  \multicolumn{1} { | c | }{$r$= 0.375}  &  \multicolumn{1} { | c | }{$r$= 0.25} \\
    \hline
     Mobilenetv2 & 71.87$\%$ & 71.25$\%$ & 70.44$\%$ & 68.14$\%$ &  9.55$\%$ \\
     
    Mobilenetv3 & 74.04$\%$ & 73.178$\%$ & 68.756$\%$ & 65.20$\%$ &  2.834$\%$ \\

    
     Resnet18 & 69.75$\%$ & 69.61$\%$ & 69.56$\%$ & 69.27$\%$ & 54.93$\%$ \\
    
     Resnet50 & 76.13$\%$ & 76.13$\%$ & 75.95$\%$ & 75.41$\%$ & 66.82$\%$ \\
    
     Effnetlite & 75.44$\%$ &  75.21$\%$ & 75.13$\%$ & 47.59$\%$ & 6.356$\%$ \\
    
     Deeplabv3-mobilenetv3 & 0.6887 &  0.6773 & 0.5784  & 0.5349 & 0.19 \\

    \hline
    \multicolumn{6} { | c | }{Mixed Precision Quantization based on compression ratio}\\
    \hline
    \multicolumn{1} { | c | }{Model} & \multicolumn{1} { | c | }{FP32} &  \multicolumn{4}{|c|}{Relative BOPs wrt W8A16 ($r$)} \\
    \hline
    Model & FP32 & $r$= 0.75 & $r$= 0.5 & $r$= 0.375 & $r$= 0.25\\
    \hline
     Mobilenetv2 & 71.87$\%$ & 71.22$\%$ & 70.69$\%$ & 69.47$\%$ &  64.65$\%$ \\
    
     Resnet18 & 69.75$\%$ & 69.60$\%$ & 69.53$\%$ & 69.30$\%$ & 69.13$\%$ \\
    
     Resnet50 & 76.13$\%$ & 76.08$\%$ & 75.77$\%$ & 75.64$\%$ & 75.17$\%$ \\
    
     Effnetlite & 75.44$\%$ &  75.25$\%$ & 75.24$\%$ & 74.84$\%$ & 68.44$\%$ \\
    
    \hline
    Model & FP32 & $r$= 0.54 & $r$= 0.5 & $r$= 0.32 & $r$= 0.25\\
    \hline

     Deeplabv3-mobilenetv3 & 0.6887 &  0.674 & 0.667 & 0.666 & 0.558 \\
     \hline
    
\end{tabular}
    \caption{Compression budget based mixed precision using W4A8, W8A8 and W8A16 bitwidth candidates obtained using our AdaRound integrated mixed precision algorithm}
    \label{tab:my_label}
\end{table}

\subsection{Phase 2 runtime comparison}
In this section, we compare the overall time taken by the sequential and interpolation search based phase 2 to return the least BOPs model that meet the desired performance budget. Table 2 shows time taken by these two schemes to find a mixed precision configuration based on task performance budget.


\begin{table}[H]
    \addtolength{\tabcolsep}{-2pt}
    \fontsize{7pt}{7pt}\selectfont
    \centering
    \begin{tabular}{ || c c c c || }
    \hline
    Model & Target & Sequantial Search & Interpolation Search \\ [0.5 ex]
    \hline \hline
    Efficientnet lite & $74.4\%$ & 2.3 hours & 1 hours \\
    Efficientnet lite & $70.4\%$ & 4.4 hours & 2.2 hours \\
    Deeplabv3+ & 0.719 & 1 hours & 0.5 hours \\
    Deeplabv3+ & 0.679 & 9.5 hours & 3.2 hours \\
    \hline
    \end{tabular}
    \caption{Runtime comparison between sequential and interpolation based search for phase 2}
    \label {table:1}
\end{table}


\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.23\textwidth]{figures/Mobilenetv3_4_8_16_pareto.png}} 
    \subfigure{\includegraphics[width=0.23\textwidth]{figures/Deeplabv3 Mobilenetv3 backbone_4_8_16_pareto.png}} 
    \caption{ W4A8, W8A8, W8A16 mixed precision and fixed precision quantization comparison for (Left) Mobilenetv3 (Right) Deeplabv3-mobilenetv3 backbone}
\end{figure}


\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.46\textwidth]{figures/efficientnet_lite0_cand4_pareto.png}} 
    \subfigure{\includegraphics[width=0.46\textwidth]{figures/mobilenetv2_cand4_pareto.png}} 
    \caption{(Top) W4A6, W6A6, W6A8, W8A8 mixed precision quantization for Efficientnet lite (Bottom) W4A4, W4A6, W6A4, W6A6, W8A6, W6A8, W8A8, W8A16 mixed precision quantization for Mobilenetv2}
\end{figure}


 

% \end{@twocolumnfalse}]

% \twocolumn[
% \begin{@twocolumnfalse}

% \end{@twocolumnfalse}]


==> sections/05_experiments.tex <==
\section{Experiments}
In this section we conduct experiments on various models to evaluate the performance of our method in different mixed precision settings. We start with defining our experimental setup by describing the datasets and the networks, compare our mixed precision results to fixed precision quantization results and finally discuss various ablations to understand the benefits of our algorithm. 

\subsubsection{Datasets:} For our experiments, we use the Imagenet-1K \cite{russakovsky2015imagenet}, MS-COCO, Pascal VOC dataset \cite{everingham2015pascal} and GLUE benchmark \cite{wang2018glue}. Due to post training nature of the algorithm, no training or finetuning is involved. Standard dataset based inference time augmentation pre-processing is used on the images.

\subsubsection{Network:} We evaluate our algorithm on ResNet18, ResNet50 \cite{he2016deep}, Mobilenetv2 \cite{sandler2018mobilenetv2}, Efficientnet-lite \cite{tan2019efficientnet}, Mobilenetv3, Deeplabv3-mobilenetv3 backbone, and BERT model . We do not fix pre-defined bitwidths for any layers or activations and include the entire network in the mixed precision search space.

\subsection{Robustness to Data Variation}
In this section, we address challenges of obtaining an accurate sensitivity list and its dependency on quality and quantity available for Phase 1. An alternate way of measuring sensitivity in phase 1 is through calculating the degradation in task performance with respect to full precision network. However, such an approach can be computational very expensive due to multiple evaluations on the validation set and greatly depends on the quality and quantitity of validation dataset used to obtain a sensitivity list. 

To understand this problem, we conduct ablation studies on Mobilenetv2 network and bitwidth candidates W4A8 and W8A8 as our mixed precision search space. We define the sensitivity list obtained using the entire 50K Imagenet validation images during phase 1 as our ground truth sensitivity list as this is the best possible sensitivity list we can obtain in post training setting. We choose 5 random subsets of 256 Imagenet images and use these subsets to obtain the sensitivity list and its corresponding phase 2 pareto curve which is the accuracy of the mixed precision network evaluated on full validation set vs relative BOPs with respect to baseline candidate.

As shown in Figure \ref{fig:fig1}, the pareto curve obtained in phase 2 with accuracy metric is greatly affected by the quality of images used to created the sensitivity list. With the same experimental setting, SQNR achieves a more optimum pareto curve and a much smaller variation with variation in data. This makes SQNR metric more reliable for a hyper-parameter free mixed precision approach for practical usecase.
\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.23\textwidth]{figures/mobilenetv2_robust_acc.png}} 
    \subfigure{\includegraphics[width=0.23\textwidth]{figures/mobilenetv2_robust_sqnr.png}} 



    \caption{Pareto fronts obtained using full Imagenet validation set and 5 random subsets of 256 Imagenet images in Phase 1 using \textbf{Left:} accuracy \textbf{Right:} SQNR }
    \label{fig:fig1}
\end{figure}

\subsection{Variation with number of images}
To understand the importance of numbers of images used for obtaining the sensitivity list, we conduct ablation to quantify the quality of sensitivity list obtained using different number of images for accuracy and SQNR metric. In figure 2, we plot the Kendal-Tau correlation coefficient between the sensitivity list obtained for each experimental setting with respect to the ground truth sensitivity list. As shown in the figure, in low data post training regime, SQNR metric is much more stable and outperforms accuracy metric to obtain a more accurate sensitivity list. As number of images increases, accuracy metric outperforms SQNR and achieves more optimum pareto curve closer to the ground truth whereas with SQNR, even with 256 images, we obtain a pareto curve very close to ground truth pareto.

\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.20\textwidth]{figures/ktau_mobilenetv2.png}} 
    \subfigure{\includegraphics[width=0.20\textwidth]{figures/mbnetv2_accuracy.png}}         \subfigure{\includegraphics[width=0.20\textwidth]{figures/ktau_resnet50.png}} 
    \subfigure{\includegraphics[width=0.20\textwidth]{figures/resnet50_accuracy.png}} 

    \caption{W4A8 and W8A8 mixed precision experiments. (Left) K-Tau correlation coefficient between sensitivity lists obtained using accuracy and SQNR metric and ground truth sensitivity list for (top) Mobilenetv2 (bottom) Resnet50 (Right) Pareto comparison between multiple accuracy based mixed precision schemes for (top) Mobilenetv2 (bottom) Resnet50 }
    \label{fig:fig2}
\end{figure}
\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.23\textwidth]{figures/mobilenetv2_MSCOCO.png}} 
    \subfigure{\includegraphics[width=0.23\textwidth]{figures/efficientnet_lite_MSCOCO.png}} 

    \caption{W4A8 and W8A8 mixed precision using MSCOCO data for \textbf{Left:}  Mobilenetv2 \textbf{Right:}  Efficientnet lite}
    \label{fig:fig3}
\end{figure}

\subsection{Capturing sensitivity using SQNR vs other metrics}
Due to the discretized nature of accuracy metric in presence of less data, the quality of the accuracy based sensitivity list greatly depends on good representativeness the dataset used in Phase 1. SQNR being a softer metric captures the relative sensitivity of layers to quantization better specially in low data regime. In this section, we conduct ablations to understand how SQNR compares to other soft metrics such as cross entropy and MSE by plotting the per image metric variation for each quantizer in the network. As shown in figure 4, we can observe that SQNR metric is more expressive and captures the relatively sensitivity more distinctively than cross entropy and MSE, which explains its effectiveness in obtaining an accurate sensitivity list even with as less as using 256 images. 

\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.4\textwidth]{figures/mobilenetv2_sqnr.png}} 
    \subfigure{\includegraphics[width=0.4\textwidth]{figures/mobilenetv2_xent.png}}         \subfigure{\includegraphics[width=0.4\textwidth]{figures/mobilenetv2_mse.png}} 

    \caption{Box plot showing per image metric variation using 256 images for each quantizer (Top) SQNR (Center) Cross Entropy (Bottom)  MSE}
    \label{fig:fig2}
\end{figure}

\subsection{Label Free Mixed Precision}
In many of practical use cases, the user doesn't have access to enough or any training or validation data for the task due to privacy reasons. As described in the previous sections, labels have no role during phase 1 of our algorithm. This opens up possibility to use similar task domain data to perform mixed precision analysis in such scenario. In this section, we use 256 MS-COCO images during both phases of our algorithm both for quantization range setting and sensitivity list creation. Even without any task data (imagenet images) used during phase 1, we find the pareto curves obtained in phase 2 for Mobilenetv2 and Efficientnet lite [figure \ref{fig:fig3}] are very similar to the ground truth pareto curves obtained using full Imagenet validation data.

\subsection{AdaRound integrated Mixed Precision}
We propose two schemes to interweave AdaRound with the mixed precision pipeline. The first scheme uses stitching of AdaRounded weights to improve the performance of mixed precision networks in Phase 2. The second scheme involves integrating AdaRounded weights in both phases of the algorithm. Specially for low bit quantization, it is important to consider the effect of AdaRounded weights while creating the sensitivity list to correctly compensate for adarounded weight-activation quantization tradeoff. 

We conduct ablation studies on Mobilenetv2 considering combinations of 4, 6, 8 and 16 bitwidths for weights and activations. In figure \ref{fig:fig4}, we can see that SQNR based mixed precision with 256 images in phase 1 performs equally good as accuracy based mixed precision with full Imagenet validation set used in phase 1. Also, both adaround interweaving schemes outperform vanilla mixed precision by achieving better validation accuracy specially in very low relative BOPs range. Interweaving AdaRound in both phases leads to a more smoother and optimum pareto curve than just interweaving AdaRound in phase 2. 
\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.40\textwidth]{figures/mobilenetv2_adaround.png}} 

    \caption{ W4A4, W4A6, W6A4, W6A6, W8A6, W6A8, W8A8 and W8A16 mixed precision ablation for Mobilenetv2. Full validation set was used in accuracy based phase 1 (orange), 256 images were used in all SQNR based phase 1 (other schemes)}
    \label{fig:fig4}
\end{figure}

% \begin{figure}[H]
%     \centering
%     \subfigure{\includegraphics[width=0.23\textwidth]{figures/efficienetnet_lite_adaround.png}} 
%     \subfigure{\includegraphics[width=0.23\textwidth]{figures/efficienetnet_lite_adaround_48.png}} 

%     \caption{ Efficientnet-lite mixed precision ablation \textbf{Left:} W4A6, W6A6, W6A8, W8A8 mixed precision ablation \textbf{Right:} W4A8 and W8A8 mixed precision ablation }
%     \label{fig:fig5}
% \end{figure}

==> sections/05_experiments_restructured.tex <==
\section{Experiments and Results}

In this section we evaluate the performance of our method on various models in different mixed precision settings. We start with defining our experimental setup by describing the datasets and the networks used, compare our mixed precision results to fixed precision quantization results and finally discuss various ablations to understand the benefits of our algorithm. 

% \begin{table*}
%     % \addtolength{\tabcolsep}{-2pt}
%     \fontsize{10.5pt}{10.5pt}\selectfont 
%     \centering
%     \begin{tabular} { | p {4 cm} | p {1 cm} | p {2 cm} |p {2.5 cm} |p {1.5 cm} | p {2.5 cm} | }
    
%     \hline
%     Model & FP32 & W8A8 ($r$=0.5) &  Mixed Precision ($r$=0.5) &  W6A8 ($r$=0.375) &  Mixed Precision ($r$=0.375)\\
%     \hline
%     % \multicolumn{2} { | c | }{Rel. BOPs wrt W8A16 (r) } &  \multicolumn{1} { | c | }{$r$= 1}  &  \multicolumn{1} { | c | }{$r$= 0.5}  &  \multicolumn{1} { | c | }{$r$= 0.375}  &  \multicolumn{1} { | c | }{$r$= 0.25} \\
%     % \hline:q
     
%     Mobilenetv3 & $74.04\%$ & $68.75\%$ & $71.65\%$ &$65.20\%$ &  $66.70\%$ \\

%     Deeplabv3-mobilenetv3 & $0.6887$ &  $0.5784$ & $0.6700$ & $0.535$ & $0.669$ \\

%     Efficientnet-lite & $75.44\%$ &  $75.13\%$ & $75.14\%$ & $73.43\%$ & $73.64\%$\\

%     Mobilenetv2 & $71.87\%$ & $70.44\%$ & $70.68\%$ & $68.14\%$ &  $67.38\%$\\

%     Resnet50 & $76.13\%$ & $75.95\%$ & $75.95\%$ & $75.41\%$ & $74.98\%$\\

%     Resnet18 & $69.75\%$ & $69.56\%$ & $69.56\%$ & $69.27\%$ & $67.39\%$\\
    

%     \hline

% \end{tabular}
%     \caption{Mixed precision using W4A8, W8A8 and W8A16 bit-width candidates. Comparison between fixed precision quantization and mixed precision quantization}
%     \label{tab:fixed-vs-mixed}
% \end{table*}

% \begin{table*}
%     % \addtolength{\tabcolsep}{-2pt}
%     \fontsize{10.5pt}{10.5pt}\selectfont 
%     \centering
%     \begin{tabular} { | p {4 cm} | p {1 cm} | p {2 cm} |p {2.5 cm} |p {1.5 cm} | p {2.5 cm} | }
%     \hline
%     Model & FP32 & W6A6 ($r$=0.281) & Mixed Precision ($r$=0.281) &  W4A8 ($r$=0.25)  &  Mixed Precision ($r$=0.25)\\
%     \hline
%     % \multicolumn{2} { | c | }{Rel. BOPs wrt W8A16 (r) } &  \multicolumn{1} { | c | }{$r$= 1}  &  \multicolumn{1} { | c | }{$r$= 0.5}  &  \multicolumn{1} { | c | }{$r$= 0.375}  &  \multicolumn{1} { | c | }{$r$= 0.25} \\
%     % \hline
     
%     Mobilenetv3 & $74.04\%$ & $4.19\%$ & $42.57\%$  & $2.83\%$ & $28.67\%$ \\

%     Efficientnet-lite & $75.44\%$ &  $72.87\%$ & $74.17\%$ & $6.37\%$ & $73.49\%$\\

%     Mobilenetv2 & $71.87\%$ & 58.60$\%$ & $64.97\%$ & $9.55\%$ &$61.81\%$ \\

%     Resnet50 & $76.13\%$ & $70.54\%$ & $73.11\%$ & $66.82\%$ & $73.05\%$\\

%     Resnet18 & $69.75\%$ & $66.09\%$ & $65.14\%$ & $54.93\%$ & $63.14\%$\\
    

%     \hline

% \end{tabular}
%     \caption{Compression budget based mixed precision using expanded search space: W4A4, W4A6, W6A4, W6A6, W8A6, W6A8, W8A8, W8A16 bit-width candidates. Comparison between fixed precision quantization and mixed precision quantization for low bit-widths}
%     \label{tab:fixed-vs-mixed_expanded}
% \end{table*}


\subsubsection{Datasets:} For our experiments, we use the Imagenet-1K \cite{russakovsky2015imagenet}, Pascal VOC dataset \cite{everingham2015pascal} and GLUE benchmark \cite{wang2018glue}. Due to post-training nature of the algorithm, no training or fine-tuning is involved. Standard dataset based inference time augmentation pre-processing is used on the images.



% \begin{figure*}
% \centering
%     \subfigure{}{\includegraphics[width=0.20\textwidth]{figures/Mobilenetv3_4_8_16_pareto_withoutadaround.png} }
%     \subfigure{\includegraphics[width=0.20\textwidth]{figures/deeplabv3_mobilenetv3_4_8_16_pareto_withoutadaround.png}} 
%     \subfigure{\includegraphics[width=0.20\textwidth]{figures/efficientnet_lite0_4_8_16_pareto_withoutadaround.png}} 
    
%     \subfigure{\includegraphics[width=0.28\textwidth]{figures/mobilenetv2_cand4_pareto_withoutadaround.png}} 
%     \subfigure{\includegraphics[width=0.28\textwidth]{figures/mobilenetv2_cand4_pareto_withoutadaround.png}} 

%     \caption{\textbf{Top:} Mixed Precision with W4A8, W8A8, W8A16 bit-widths for Mobilenetv3, Deeplabv3-mobilenetv3 backbone and Efficientnet lite \textbf{Bottom:} Mixed Precision with W4A4, W4A6, W6A4, W6A6, W8A6, W6A8, W8A8, W8A16 bit-widths for Mobilenetv2 and Efficientnet lite}
%     \label{fig:fig1}
% \end{figure*}


\begin{figure*}
    \centering
    \subfigure{\includegraphics[width=0.30\textwidth]{figures/mobilenetv2_robust_acc.pdf}} 
    \subfigure{\includegraphics[width=0.30\textwidth]{figures/mobilenetv2_robust_sqnr.pdf}} 
    \subfigure{\includegraphics[width=0.30\textwidth]{figures/ktau_mobilenetv2.pdf}} 
    % \subfigure{\includegraphics[width=0.23\textwidth]{figures/mbnetv2_accuracy.png}}        
    
    %\subfigure{\includegraphics[width=0.18\textwidth]{figures/ktau_resnet50.png}} 
    % \subfigure{\includegraphics[width=0.18\textwidth]{figures/resnet50_accuracy.png}} 

    \caption{Variation in pareto curves obtained using different subsets of 256 Imagenet images using \textit{Left:} Accuracy \textit{Center:} SQNR metric in Phase 1 to measure per-layer quantization sensitivity. \textit{Right:} Kendall-Tau co-relation coefficient ($\tau$) of the sensitivity list obtained using SQNR and accuracy metric using different number of Imagenet images with ground-truth sensitivity list.}
    \label{fig:ktau}
\end{figure*}


\subsubsection{Network:} We evaluate our algorithm on ResNet18, ResNet50 \cite{he2016deep}, Mobilenetv2 \cite{sandler2018mobilenetv2}, Efficientnet-b0, Efficientnet-lite \cite{tan2019efficientnet}, Mobilenetv3 \cite{howard2019searching}, Deeplabv3-mobilenetv3 \cite{chen2017rethinking}, BERT and ViT model \cite{devlin2018bert}. 

For our experiments, we use the AI Model Efficiency Toolkit (AIMET) \cite{aimet,siddegowda2022neural} to quantize the models to desired bit-widths and use the per-channel weight quantization and symmetric and asymmetric schemes for weight and activation tensors, respectively. We set the quantization range of each quantizer using an MSE based criteria~\cite{nagel2021white}. We do not fix pre-defined bit-widths for any layers or activations in the mixed precision search space and report all mixed precision results in terms of relative BOPs ($r$) with respect to fixed W8A16 representation for each model.



\subsection{Comparison to Fixed Precision Quantization}
Some networks are very sensitive to quantization due to the presence of layers with large activation ranges with outliers. These ranges are difficult to represent accurately in fixed precision representation. For networks with this issue, mixed precision quantization can be very useful to achieve a better performance-efficiency trade-off by representing problematic layers in high precision while keeping rest of the network in lower bit-widths. 

In Table \ref{tab:fixed-vs-mixed} and \ref{tab:BERT}, we summarize our PTQ mixed precision results using a practical bit-width search space with frequently available bit-widths (W4A8, W8A8 and W8A16) for on-device deployment. We notice that for problematic networks like Mobilenetv3, Deeplabv3, Efficientnet, BERT and ViT, mixed precision quantization outperform its equivalent single precision quantized networks by automatically finding problematic layers and keeping them in higher bits to achieve better performance-efficiency trade-off. 
To understand better why some networks benefit more from mixed precision than others, we visualize the per-layer quantization sensitivity of all networks in Figure \ref{fig:sqnr-range}.
%A comparative behavior of different networks is summarized in figure \ref{fig:sqnr-range}. 
Networks which have layers with outliers like BERT, ViT, Deeplabv3 and Mobilenetv3 exhibit a large SQNR range and have some activations achieving very low SQNR values suggesting significant difference in sensitivity to quantization among layers in these networks. On the contrary, for networks like Resnet18 and Resnet50, we observe a much smaller range of higher SQNR values which explains why mixed precision is less useful for such networks, as many layers have a similar quantization sensitivity. We expect to see in our results that mixed precision works well for the former group, and does not improve significantly on the second group. 



\begin{table}
    % \addtolength{\tabcolsep}{-2pt}
    \centering
    \begin{tabular} {  lccccc }
    \toprule
    Task & FP32 & W8A8 ($r$=0.5) &  PTQ MP ($r$=0.5) \\
    \midrule
    RTE & $68.23$ & $49.82$ & $67.14$ \\
    MRPC & $90.38$ & $71.40$ & $86.44$ \\
    SST-2 & $92.43$ & $85.78$ & $91.39$ \\
    STS-B & $88.61$ & $80.63$ & $87.69$ \\
    MNLI & $84.40$ & $74.13$ & $82.97$ \\
    \bottomrule
\end{tabular}
    \caption{MPQ results using W4A8, W8A8, W8A16 bit-width candidates for BERT.}
    \label{tab:BERT}
\end{table}



% \begin{table*}
%     % \addtolength{\tabcolsep}{-2pt}
%     \centering
%     \begin{tabular} {  lccccc }
%     \toprule
%     Model & FP32 & PTQ MP &  AdaRound integrated MP &  PTQ MP & AdaRound integrated MP \\
%     &   &  ($r$=0.50) &  ($r$=0.50) &   ($r$=0.375)  &  ($r$=0.375)\\

%     \midrule
%     Resnet18 & $69.75\%$ & $69.56\%$ & $69.56\%$ & $67.39\%$ & $69.30\%$\\
%     Resnet50 & $76.13\%$ & $75.95\%$ & $75.95\%$ & $74.98\%$ & $75.64\%$\\\
%     Efficientnet-lite & $75.44\%$ &  $75.14\%$ & $75.24\%$ & $73.64\%$ & $74.84\%$\\
%     Mobilenetv2 & $71.87\%$ & $70.68\%$ & $70.69\%$ & $67.38\%$ &  $69.47\%$\\
%     Mobilenetv3 & $74.04\%$ & $71.65\%$ & $72.66\%$ &$66.70\%$ &  $71.26\%$ \\
%     Deeplabv3-mobilenetv3 & $0.6887$ &  $0.6700$ & $0.6670$ & $0.6690$ & $0.6692$ \\
%     \bottomrule
% \end{tabular}
%     \caption{Comparison between PTQ MP and AdaRound integrated MP for W4A8,W8A8, W8A16 search space.}
%     \label{tab:vanilla-vs-adarounded}
% \end{table*}

\begin{table*}
    % \addtolength{\tabcolsep}{-2pt}
    \centering
    \begin{tabular} {  lccccc }
    \toprule
    Model & FP32 & W8A8 AdaRound & MP AdaRound &  W6A8 AdaRound & MP AdaRound\\
    &   &  ($r$=0.50) &  ($r$=0.50) &   ($r$=0.375)  &  ($r$=0.375)\\

    \midrule
    Resnet18 & $69.75\%$ & $69.54\%$ & $69.68\%$ & $69.53\%$ & $69.53\%$\\
    Resnet50 & $76.13\%$ & $75.96\%$ & $75.96\%$ & $75.82\%$ & $75.91\%$\\
    Efficientnet-lite & $75.44\%$ &  $75.34\%$ & $75.36\%$ & $75.23\%$ & $75.18\%$\\
    Efficientnet-b0 & $77.67\%$ &  $14.98\%$ & $76.55\%$ & $12.67\%$ & $69.78\%$\\
    Mobilenetv2 & $71.87\%$ & $70.62\%$ & $70.98\%$ & $70.51\%$ &  $70.56\%$\\
    Mobilenetv3 & $74.04\%$ & $69.96\%$ & $72.83\%$ &$69.76\%$ &  $71.40\%$ \\
    Deeplabv3-Mobilenetv3 & $0.6887$ &  $0.5865$ & $0.6708$ & $0.5827$ & $0.6692$ \\
    \bottomrule
\end{tabular}
    \caption{Comparison between fixed precision AdaRound and MP AdaRounded models for W4A8, W6A8, W8A8, W8A16 search space.}
    \label{tab:vanilla-vs-adarounded}
\end{table*}

Further, to demonstrate generality of our method to lower weight and activation bit-widths, we perform mixed precision analysis on an expanded search space by including 4 and 6 bit quantization for weight and activation tensors. The results are summarized in Table \ref{tab:fixed-vs-mixed_expanded}. Our Mixed precision quantization routine is able to significantly improve accuracy of the networks specially in lower BOPs models by rightly identifying sensitive layers and assigning higher bit-widths to them.

% We also expand our search space to 6 and 4 bits for weights and activations and compare our mixed precision algorithm to fixed precision quantization. In most usecases, at a similar relative BOPs value,
% our mixed precision solution outperforms or performs at par with single precision quantized network achieving a better performance-latency tradeoff.

% \begin{table*}
%     % \addtolength{\tabcolsep}{-2pt}
%     \fontsize{10.5pt}{10.5pt}\selectfont 
%     \centering
%     \begin{tabular} { | p {3.6 cm} | p {1.3 cm} | p {1.5 cm} |p {4 cm} |p {1.4 cm} | p {4 cm} | }
    
%     \hline
%     Model & FP32 & PTQ MP ($r$=0.5) &  AdaRound integrated MP ($r$=0.5) &  PTQ MP ($r$=0.375) & AdaRound integrated MP ($r$=0.375)\\
%     \hline
%     % \multicolumn{2} { | c | }{Rel. BOPs wrt W8A16 (r) } &  \multicolumn{1} { | c | }{$r$= 1}  &  \multicolumn{1} { | c | }{$r$= 0.5}  &  \multicolumn{1} { | c | }{$r$= 0.375}  &  \multicolumn{1} { | c | }{$r$= 0.25} \\
%     % \hline:q
     
%     Mobilenetv3 & $74.04\%$ & $71.65\%$ & $-\%$ &$66.70\%$ &  $-\%$ \\

%     Deeplabv3-mobilenetv3 & $0.6887$ &  $0.6700$ & $0.667$ & $0.6690$ & $0.6692$ \\
    
%     Efficientnet-lite & $75.44\%$ &  $75.14\%$ & $75.24\%$ & $73.64\%$ & $74.84\%$\\

%     Mobilenetv2 & $71.87\%$ & $70.68\%$ & $70.69\%$ & $67.38\%$ &  $69.47\%$\\

%     Resnet50 & $76.13\%$ & $75.95\%$ & $75.95\%$ & $74.98\%$ & $75.64\%$\\

%     Resnet18 & $69.75\%$ & $69.56\%$ & $69.56\%$ & $67.39\%$ & $69.30\%$\\
    
%     \hline
% \end{tabular}
%     \caption{Comparison between PTQ MP and AdaRound integrated MP for W4A8,W8A8, W8A16 search space.}
%     \label{tab:vanilla-vs-adarounded}
% \end{table*}




% \subsection{Robustness to Quality and Quantity of data used for Phase 1}
% % Obtaining an accurate sensitivity list is very crucial as it directly guides the performance drop vs BOPs gain tradeoff at each step of our Phase 2. In this section, we address challenges of obtaining an accurate sensitivity list and its dependency on quality and quantity available for Phase 1. 
% An alternate way of capturing the quantization sensitivity of a layer is to measure the degradation in task performance with respect to full precision network upon quantization of that layer. Such a surrogate measure of the relative effect of quantization on different layers works well however it can be computationally expensive due to multiple evaluations on the validation set. Also, the accuracy of such a sensitivity list is affected by how well representative the validation set was of the overall data distribution. To investigate this, we choose 5 random subsets of 256 Imagenet images and use these subsets to obtain the quantization sensitivity list using the accuracy and SQNR metric. As we observe in Figure \ref{fig:ktau}, the pareto curve obtained with accuracy metric drastically varies with choice of the subset of images used to creating the sensitivity list. With the same experimental settings, SQNR achieves a much smaller variation in the pareto curve obtained using different subsets of data. 

% Next, we study the effect of using more images on the accuracy of sensitivity list obtained in Phase 1. To quantify the quality of the sensitivity list obtained using different of number of images, we use the Kendall Tau correlation coefficient between the obtained sensitivity list and the ground truth sensitivity list which we define as sensitivity list obtained using measuring the accuracy degradation on the entire 50K Imagenet validation set as a surrogate measure. Due to the discrete nature of the accuracy metric in presence of less data, the accuracy metric is not able to correctly capture the relative sensitivity of layers to quantization. In similar settings, SQNR being a softer metric captures the relative sensitivity of layers to quantization better leading to higher Kendall Tau score.

% In conclusion, using SQNR to measure the sensitivity of layers to quantization shows both advantages - robustness to number and variation in data used for Phase 1, making it a reliable choice for a hyper-parameter free mixed precision approach for practical use-cases.

% % \begin{figure*}
% %     \centering
% %     \subfigure{\includegraphics[width=0.32\textwidth]{figures/mobilenetv2_robust_acc.png}} 
% %     \subfigure{\includegraphics[width=0.32\textwidth]{figures/mobilenetv2_robust_sqnr.png}} 
% %     \subfigure{\includegraphics[width=0.32\textwidth]{figures/ktau_mobilenetv2.png}} 
% %     % \subfigure{\includegraphics[width=0.23\textwidth]{figures/mbnetv2_accuracy.png}}        
    
% %     %\subfigure{\includegraphics[width=0.18\textwidth]{figures/ktau_resnet50.png}} 
% %     % \subfigure{\includegraphics[width=0.18\textwidth]{figures/resnet50_accuracy.png}} 

% %     \caption{Pareto fronts obtained using full Imagenet validation set and 5 random subsets of 256 Imagenet images in Phase 1 using \textbf{Left:} accuracy \textbf{Right:} SQNR }
% %     \label{fig:ktau}
% % \end{figure*}


% % However, such an approach can be computational very expensive due to multiple evaluations on the validation set and greatly depends on the quality and quantitity of validation dataset used to obtain a sensitivity list. 

% % To understand this problem, we conduct ablation studies on Mobilenetv2 network with bit-width candidates W4A8 and W8A8 as our mixed precision search space. We define the sensitivity list obtained using measuring the accuracy on the entire 50K Imagenet validation images during phase 1 as our ground truth sensitivity list as this is the best possible sensitivity list we can obtain in post-training setting. We choose 5 random subsets of 256 Imagenet images and use these subsets to obtain the sensitivity list and its corresponding phase 2 pareto curve.



% % Another way to reduce the dependency on the quality of images used for creating the sensitivity list is to increase the number of images used for phase 1. However, using more images increases the overall runtime due to increased validation subset. To understand the importance of numbers of images used for obtaining the sensitivity list, we quantify the quality of sensitivity list obtained using different number of images for both accuracy and SQNR metric using the Kendall Tau Rank correlation coefficient. In figure \ref{fig:ktau}, we plot the Kendal-Tau correlation coefficient between the sensitivity list obtained for each experimental setting with respect to the ground truth sensitivity list. As shown in the figure, in low data post-training regime, SQNR metric is much more stable and outperforms accuracy metric to obtain a more accurate sensitivity list. As the number of images increases, accuracy metric based mixed precision improves and obtains more optimum pareto front in phase 2.

% % Hence, using SQNR to measure the sensitivity of quantizers to quantization shows both advantages - robustness to number and variation of data used for Phase 1, making it a reliable choice for a hyper-parameter free mixed precision approach for practical use cases.

% % \begin{figure}
% %     \centering
% %     \subfigure{\includegraphics[width=0.20\textwidth]{figures/ktau_mobilenetv2.png}} 
% %     \subfigure{\includegraphics[width=0.20\textwidth]{figures/mbnetv2_accuracy.png}}         \subfigure{\includegraphics[width=0.20\textwidth]{figures/ktau_resnet50.png}} 
% %     \subfigure{\includegraphics[width=0.20\textwidth]{figures/resnet50_accuracy.png}} 

% %     \caption{W4A8 and W8A8 mixed precision experiments. (Left) K-Tau correlation coefficient between sensitivity lists obtained using accuracy and SQNR metric and ground truth sensitivity list for (top) Mobilenetv2 (bottom) Resnet50 (Right) Pareto comparison between multiple accuracy based mixed precision schemes for (top) Mobilenetv2 (bottom) Resnet50 }
% %     \label{fig:ktau}
% % \end{figure}


% % \subsection{Capturing sensitivity using SQNR vs other metrics}
% % Due to the discretized nature of accuracy metric in presence of less data, the quality of the accuracy based sensitivity list highly depends on good representativeness the dataset used for Phase 1. SQNR being a softer metric captures the relative sensitivity of layers to quantization better in similar experimental settings. In this section, we compare SQNR to other soft metrics such as cross entropy and MSE by plotting the per image metric variation for each quantizer in the network. As shown in figure \ref{fig:metric-ablation}, we can observe that SQNR metric is more expressive and captures the relatively sensitivity more distinctively than cross entropy and MSE, which explains its effectiveness in obtaining an accurate sensitivity list even with 256 images. 





% \subsection{Label Free Mixed Precision}
% In many of practical use cases, the user doesn't have access to enough or any training or validation data for the task due to privacy reasons. As described in the previous sections, labels have no role during phase 1 of our algorithm. This opens up possibility to use similar task domain data to perform mixed precision analysis in such scenario. To demonstrate this, we use 256 MS-COCO images during both phases of our algorithm for quantization range setting and sensitivity list creation. Even without any task data (Imagenet images) used, we find the pareto curves obtained in phase 2 for Mobilenetv2 and Efficientnet lite [figure \ref{fig:label-free}] are very similar to pareto curve obtained using Imagenet images in similar experimental settings.




% \begin{figure}
%     \centering
%     \subfigure{\includegraphics[width=0.23\textwidth]{figures/mobilenetv2_MSCOCO.png}} 
%     \subfigure{\includegraphics[width=0.23\textwidth]{figures/efficientnet_lite_MSCOCO.png}} 

%     \caption{Comparison between MP performed using out-of-task data (MS-COCO images) and task-data (Imagenet images) for \textit{Left:}  Mobilenetv2 \textit{Right:}  Efficientnet-lite. Both scenarios achieve similar performance-compression trade-off.}
%     \label{fig:label-free}
% \end{figure}

\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.42\textwidth]{figures/SQNR_W8.pdf}} 

    \caption{Range of SQNR values for W8A8 quantizers in different networks. Networks with layers with outliers or irregular distributions exhibit large SQNR range due to difference in sensitivity of layers to quantization.}
    \label{fig:sqnr-range}
\end{figure}


\subsection{Robustness to Calibration Data}
Calibration data plays an important role in most post-training quantization algorithms to estimate quantization range settings for activation feature maps of a network. At times, using an under representative calibration set for PTQ methods can lead to sub-optimum performance, making it challenging to adapt for practical use-cases where little or no task data is available. In this section, we discuss robustness of our algorithm to variation in calibration data used for performing mixed precision, highlighting the wide applicability of our method for real-world scenarios.

\subsubsection{Robustness to variation in images} In order to understand the advantage of using SQNR as a metric to capture per-layer quantization sensitivity, we compare SQNR with other surrogate metrics. 
An alternate way of capturing the quantization sensitivity of a layer is to measure the degradation in task performance with respect to full precision network upon quantization of that layer. Such a surrogate measure of the relative effect of quantization on different layers works well however it can be computationally expensive due to multiple evaluations on the validation set. Also, the accuracy of such a sensitivity list is affected by how well representative the validation set was of the overall data distribution. To investigate this, we use 5 random subsets of 256 Imagenet images to obtain the quantization sensitivity list using the accuracy and SQNR metric. As we observe in Figure \ref{fig:ktau}, the pareto curve obtained with accuracy metric drastically varies with choice of the subset of images used to creating the sensitivity list. With the same experimental settings, SQNR achieves a much smaller variation in the pareto curve obtained using different subsets of data. 



\subsubsection{Robustness to numbers of images}Next, we study the effect of using more images on the accuracy of sensitivity list obtained in Phase 1. To quantify the quality of the sensitivity list obtained using different of number of images, we use the Kendall Tau correlation coefficient between the obtained sensitivity list and the ground truth sensitivity list which we define as sensitivity list obtained using measuring the accuracy degradation on the entire 50K Imagenet validation set as a surrogate measure. Due to the biased nature of the accuracy metric in presence of less or unbalanced calibration data, using accuracy measurements to capture relative sensitivity of layers to quantization can be inaccurate, hence leading to sub-optimal sensitivity list. In similar settings, SQNR being a softer metric, captures the relative sensitivity of layers to quantization better leading to higher Kendall Tau score.

% Due to the discrete nature of the accuracy metric in presence of less data, the accuracy metric is not able to correctly capture the relative sensitivity of layers to quantization. In similar settings, SQNR being a softer metric captures the relative sensitivity of layers to quantization better leading to higher Kendall Tau score.



% \begin{figure*}
%     \centering
%     \subfigure{\includegraphics[width=0.32\textwidth]{figures/mobilenetv2_robust_acc.png}} 
%     \subfigure{\includegraphics[width=0.32\textwidth]{figures/mobilenetv2_robust_sqnr.png}} 
%     \subfigure{\includegraphics[width=0.32\textwidth]{figures/ktau_mobilenetv2.png}} 
%     % \subfigure{\includegraphics[width=0.23\textwidth]{figures/mbnetv2_accuracy.png}}        
    
%     %\subfigure{\includegraphics[width=0.18\textwidth]{figures/ktau_resnet50.png}} 
%     % \subfigure{\includegraphics[width=0.18\textwidth]{figures/resnet50_accuracy.png}} 

%     \caption{Pareto fronts obtained using full Imagenet validation set and 5 random subsets of 256 Imagenet images in Phase 1 using \textbf{Left:} accuracy \textbf{Right:} SQNR }
%     \label{fig:ktau}
% \end{figure*}


% However, such an approach can be computational very expensive due to multiple evaluations on the validation set and greatly depends on the quality and quantitity of validation dataset used to obtain a sensitivity list. 

% To understand this problem, we conduct ablation studies on Mobilenetv2 network with bit-width candidates W4A8 and W8A8 as our mixed precision search space. We define the sensitivity list obtained using measuring the accuracy on the entire 50K Imagenet validation images during phase 1 as our ground truth sensitivity list as this is the best possible sensitivity list we can obtain in post-training setting. We choose 5 random subsets of 256 Imagenet images and use these subsets to obtain the sensitivity list and its corresponding phase 2 pareto curve.



% Another way to reduce the dependency on the quality of images used for creating the sensitivity list is to increase the number of images used for phase 1. However, using more images increases the overall runtime due to increased validation subset. To understand the importance of numbers of images used for obtaining the sensitivity list, we quantify the quality of sensitivity list obtained using different number of images for both accuracy and SQNR metric using the Kendall Tau Rank correlation coefficient. In figure \ref{fig:ktau}, we plot the Kendal-Tau correlation coefficient between the sensitivity list obtained for each experimental setting with respect to the ground truth sensitivity list. As shown in the figure, in low data post-training regime, SQNR metric is much more stable and outperforms accuracy metric to obtain a more accurate sensitivity list. As the number of images increases, accuracy metric based mixed precision improves and obtains more optimum pareto front in phase 2.

% Hence, using SQNR to measure the sensitivity of quantizers to quantization shows both advantages - robustness to number and variation of data used for Phase 1, making it a reliable choice for a hyper-parameter free mixed precision approach for practical use cases.

% \begin{figure}
%     \centering
%     \subfigure{\includegraphics[width=0.20\textwidth]{figures/ktau_mobilenetv2.png}} 
%     \subfigure{\includegraphics[width=0.20\textwidth]{figures/mbnetv2_accuracy.png}}         \subfigure{\includegraphics[width=0.20\textwidth]{figures/ktau_resnet50.png}} 
%     \subfigure{\includegraphics[width=0.20\textwidth]{figures/resnet50_accuracy.png}} 

%     \caption{W4A8 and W8A8 mixed precision experiments. (Left) K-Tau correlation coefficient between sensitivity lists obtained using accuracy and SQNR metric and ground truth sensitivity list for (top) Mobilenetv2 (bottom) Resnet50 (Right) Pareto comparison between multiple accuracy based mixed precision schemes for (top) Mobilenetv2 (bottom) Resnet50 }
%     \label{fig:ktau}
% \end{figure}


% \subsection{Capturing sensitivity using SQNR vs other metrics}
% Due to the discretized nature of accuracy metric in presence of less data, the quality of the accuracy based sensitivity list highly depends on good representativeness the dataset used for Phase 1. SQNR being a softer metric captures the relative sensitivity of layers to quantization better in similar experimental settings. In this section, we compare SQNR to other soft metrics such as cross entropy and MSE by plotting the per image metric variation for each quantizer in the network. As shown in figure \ref{fig:metric-ablation}, we can observe that SQNR metric is more expressive and captures the relatively sensitivity more distinctively than cross entropy and MSE, which explains its effectiveness in obtaining an accurate sensitivity list even with 256 images. 


\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.23\textwidth]{figures/mobilenetv2_MSCOCO.pdf}} 
    \subfigure{\includegraphics[width=0.23\textwidth]{figures/efficientnet_lite_MSCOCO.pdf}} 

    \caption{Comparison between MP performed using out-of-task data (MS-COCO images) and task-data (Imagenet images) for \textit{Left:}  Mobilenetv2 \textit{Right:}  Efficientnet-lite. Both scenarios achieve similar performance-efficiency trade-off.}
    \label{fig:label-free}
\end{figure}


\begin{table*}
    % \addtolength{\tabcolsep}{-2pt}
    \centering
    \begin{tabular} {  lccccc }
    \toprule
    Model & Accuracy Target & Sequential  & Binary  & Binary + Interpolation & Relative BOPs  \\         &   &  Search (hours) &  Search (hours) &   Search (hours)  & $(r)$ \\

    \midrule
    Resnet50 & $75.13\% (-1\%)$ & 12.6 & 1.6 & 1.6 & 0.396\\
    Resnet50 & $71.13\% (-5\%)$ & 14.4 & 1.6 & 1.2 & 0.257\\
    Efficientnet-lite & $74.44\% (-1\%)$ & 2.3 & 0.8 & 0.4 & 0.859\\
    Efficientnet-lite & $70.44\% (-5\%)$ & 4.4 & 0.8 & 0.5 & 0.610\\
    Mobilenetv2  & $70.89\% (-1\%)$ & 5.6 & 0.4 & 0.4 & 0.583\\
    Mobilenetv2  & $66.89\% (-5\%)$ & 8.5 & 0.8 & 0.6 & 0.365\\
    Mobilenetv3 & $73.04\% (-1\%)$ & 8.8 & 0.3 & 0.3 & 0.849\\
    Mobilenetv3 & $69.04\% (-5\%)$ & 14.1 & 0.8 & 0.4 & 0.435\\
    \bottomrule
    \end{tabular}
    \caption{Run-time comparison between sequential, binary and binary + interpolation based search for W4A8, W8A8, W8A16 MP for performance budgets: $1\%$ and $4\%$ accuracy drop from full precision accuracy. Compression achieved for obtained MP models is measured in terms of relative BOPs with respect to W8A16 model.}        \label{tab:phase2-runtime}

\end{table*}


\subsubsection{Robustness to out-of-domain data}
In many practical use-cases, the user may have access to little or no task data due to privacy reasons. As described in the previous sections, labels have no role during Phase 1 of our algorithm. This opens up possibility to use similar task domain data to perform mixed precision analysis in such scenario. To demonstrate this, we use 256 MS-COCO images during both phases of our algorithm for quantization range setting and sensitivity list creation. As summarized in Figure \ref{fig:label-free}, even without any task data (Imagenet images) used, we find the pareto curves obtained in phase 2 for Mobilenetv2 and Efficientnet lite are very similar to pareto curve obtained using Imagenet images in similar experimental settings.

In conclusion, using SQNR to measure the sensitivity of layers to quantization shows robustness to both variation and number of images in the calibration dataset, and also achieves competitive performance with similar out-of-domain data, making it a reliable choice for a hyper-parameter free mixed precision approach for practical use-cases.







\subsection{AdaRound integrated Mixed Precision}
As discussed in the previous section, the performance of low-bit quantization configurations in mixed precision can be improved by integrating AdaRound in our mixed precision routine. Integrating AdaRound in our method has no additional compute overhead other than performing AdaRound on the full precision network for each weight bit-width in the search space. To show improvements with our enhancement method we summarize comparison between fixed precision AdaRound with AdaRound integrated mixed precision in Table \ref{tab:vanilla-vs-adarounded}. Specially for low bit-width ($<$8) quantization, our AdaRound integrated mixed precision performance not only improves over fixed precision AdaRound but also outperforms its fixed precision equivalent even for quantization friendly networks like the Resnet family where mixed precision was not very helpful.

Further, to understand the advantage of interweaving AdaRound in both phases of our mixed precision routine, we conduct ablation on a Mobilenetv2 network with W4A4, W4A6, W6A4, W6A6, W8A6, W6A8, W8A8, W8A16 as our search space and compare the performance of PTQ mixed precision, AdaRound over PTQ mixed precision and AdaRound interweaved in both phases based mixed precision. As we can see in Figure \ref{fig:adaround-integration}, integrating AdaRound in both phases achieves the best performance-effiency trade-off specially in lower BOPs region signifying the importance of correctly capturing the AdaRounded weight-activation quantization trade-off for low bit activation quantization.
\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.40\textwidth]{figures/mobilenetv2_adaround.pdf}} 

    \caption{Comparison between PTQ MP, AdaRound over PTQ MP and Phase 1$\&$2 integrated AdaRound PTQ MP.}
    \label{fig:adaround-integration}
\end{figure}

% We propose two schemes to interweave AdaRound with our mixed precision pipeline. The first scheme uses stitching of AdaRounded weights to improve the performance of mixed precision networks in Phase 2. The second scheme involves integrating AdaRounded weights in both phases of the algorithm. This is important for low bit-width quantization to correctly compensate for adarounded weight-activation quantization tradeoff. 

% We conduct ablation studies on Mobilenetv2 considering combinations of 4, 6, 8 and 16 bit-widths for weights and activations. In figure \ref{fig:adaround-integration}, both AdaRound interweaving schemes outperform vanilla mixed precision by achieving better validation accuracy specially in very low relative BOPs range. Interweaving AdaRound in both phases leads to a more smoother and optimum pareto curve than just interweaving AdaRound in phase 2. 


% \begin{table*}
%     % \addtolength{\tabcolsep}{-2pt}
%     \fontsize{7.5pt}{7.5pt}\selectfont 
%     \centering
%     \begin{tabular} { | p {2 cm} | p {1 cm} | p {1.5 cm} |p {2 cm} |p {2 cm} | p {1.8 cm} | p {2 cm} | p {2.0 cm} |  p {2.1 cm} | }
    
%     \hline
%     Model & FP32 & W8A8 ($r$=0.5) &  Mixed Precision ($r$=0.5) &  AdaRound integrated Mixed Precision ($r$=0.5) & W6A8 ($r$=0.375) &  Mixed Precision ($r$=0.375) &  AdaRound integrated Mixed Precision ($r$=0.375)  \\
%     \hline
%     % \multicolumn{2} { | c | }{Rel. BOPs wrt W8A16 (r) } &  \multicolumn{1} { | c | }{$r$= 1}  &  \multicolumn{1} { | c | }{$r$= 0.5}  &  \multicolumn{1} { | c | }{$r$= 0.375}  &  \multicolumn{1} { | c | }{$r$= 0.25} \\
%     % \hline:q
     
%     Mobilenetv3 & $74.04\%$ & $68.75\%$ & $71.65\%$ & - &$65.20\%$ &  $66.70\%$ & -\\

%     Deeplabv3-mobilenetv3 & $0.6887$ &  $0.5784$ & $0.6700$ & $0.667$ & $0.535$ & $0.669$ ($r$=0.32)^{*} & $0.6692$ ($r$=0.32)^{*}\\


%     Efficientnet-lite & $75.44\%$ &  $75.13\%$ & $75.14\%$ & $75.24\%$ & $73.43\%$ & $73.64\%$ & $74.84\%$ \\

%     Mobilenetv2 & $71.87\%$ & $70.44\%$ & $70.68\%$ & $70.69\%$ & $68.14\%$ &  $67.38\%$ & $69.47\%$ \\

%     Resnet50 & $76.13\%$ & $75.95\%$ & $75.95\%$ & $75.95\%$ & $75.41\%$ & $74.98\%$ & $75.64\%$\\

%     Resnet18 & $69.75\%$ & $69.56\%$ & $69.56\%$ & $69.56\%$ & $69.27\%$ & $67.39\%$ & $69.30\%$\\
    

%     \hline

% \end{tabular}
%     \caption{Compression budget based mixed precision using W4A8, W8A8 and W8A16 bit-width candidates. Comparison between fixed precision quantization, mixed precision and AdaRound integrated mixed precision quantization}
%     \label{tab:my_label}
% \end{table*}

% \begin{table*}
%     % \addtolength{\tabcolsep}{-2pt}
%     \fontsize{7.5pt}{7.5pt}\selectfont 
%     \centering
%     \begin{tabular} { | p {2 cm} | p {1 cm} | p {1.5 cm} |p {2 cm} |p {2 cm} | p {1.8 cm} | p {2.15 cm} | p {1.95 cm} |  p {2.2 cm} | }
%     \hline
%     Model & FP32 & W6A6 ($r$=0.281) & Mixed Precision ($r$=0.281) &  W4A8 ($r$=0.25)  &  Mixed Precision ($r$=0.25) & W6A4 ($r$=0.1875) &  Mixed Precision ($r$=0.1875) \\
%     \hline
%     % \multicolumn{2} { | c | }{Rel. BOPs wrt W8A16 (r) } &  \multicolumn{1} { | c | }{$r$= 1}  &  \multicolumn{1} { | c | }{$r$= 0.5}  &  \multicolumn{1} { | c | }{$r$= 0.375}  &  \multicolumn{1} { | c | }{$r$= 0.25} \\
%     % \hline
     
%     Mobilenetv3 & $74.04\%$ & $4.19\%$ & $42.57\%$  & $2.83\%$ & $28.67\%$ &  $0.122\%$ & \\

%     Efficientnet-lite & $75.44\%$ &  $72.87\%$ & $74.17\%$ & $6.37\%$ & $73.49\%$ & $27.60\%$ & $68.89\%$ \\

%     Mobilenetv2 & $71.87\%$ & 58.60$\%$ & $64.97\%$ & $9.55\%$ &$61.81\%$ &  $0.326\%$ & $29.10\%$ \\

%     Resnet50 & $76.13\%$ & $70.54\%$ & $73.11\%$ & $66.82\%$ & $73.05\%& $4.3\%$ &$61.91\%$\\

%     Resnet18 & $69.75\%$ & $66.09\%$ & $65.14\%$ & $54.93\%$ & $63.14\%$& $13.91\%$ & $46.17\%$ \\
    

%     \hline

% \end{tabular}
%     \caption{Compression budget based mixed precision using W4A4, W4A6, W6A4, W6A6, W8A6, W6A8,
% W8A8, W8A16 bit-width candidates. Comparison between fixed precision quantization and mixed precision quantization for low bit-widths}
%     \label{tab:my_label}
% \end{table*}

% \subsection{Compression based Mixed Precision}
% Table 1 and 2 compares task performance of various mixed precision configurations of networks based on compression measured as relative BOPs with respect to W8A16 model. We compare our mixed precision algorithm with similar relative BOPs fixed precision quantized models. For all the experiments, only 256 label free task images were used both for AdaRound optimization and sensitivity calculation in phase 1, demonstrating effectiveness of our method in presence of less data.


% \begin{figure}[H]
%     \centering
%     \subfigure{\includegraphics[width=0.23\textwidth]{figures/efficienetnet_lite_adaround.png}} 
%     \subfigure{\includegraphics[width=0.23\textwidth]{figures/efficienetnet_lite_adaround_48.png}} 

%     \caption{ Efficientnet-lite mixed precision ablation \textbf{Left:} W4A6, W6A6, W6A8, W8A8 mixed precision ablation \textbf{Right:} W4A8 and W8A8 mixed precision ablation }
%     \label{fig:fig5}
% \end{figure}



\subsection{Phase 2 run-time comparison}
For task performance (accuracy) based target budgets, searching for the least BOPs model satisfying the criteria can be expensive in our trivial sequential search based phase 2. Exploiting the monotonic nature of the pareto curve, we propose to use binary search and its improved variant to improve the overall run-time of our search algorithm. Table \ref{tab:phase2-runtime} shows time taken by these three schemes to find a mixed precision configuration for desirable performance budget for absolute $1\%$ and $4\%$ drop with respect to full precision accuracy of the networks. 





==> sections/07_bibliography.tex <==
\begin{thebibliography}{9}
\bibliography{refs} % Entries are in the refs.bib file
\end{thebibliography}

